Fluctuations and correlations from NA61/SHINE

Basic ideas, methods and results related to the NA61/SHINE study of event-by-event fluctuations in high energy nuclear collisions are briefly reviewed.

==> include/Makefile <==
# Makefile for generating presentation tex related files
# $Id: Makefile 3154 2013-09-26 15:17:51Z darko $

USEPDFLATEX := 1
USEBIBTEX := 1

TARGET := na61Preprint
DEPENDENCIES := $(wildcard plots/* *.tex *.bib include/*bib)

##########################################################

LATEX := $(if $(filter 1, $(USEPDFLATEX)), pdflatex, latex)

COLORIZE := awk 'BEGIN{red="\033[31;1m";yel="\033[34m";byel="\033[34;1m";end="\033[0m"}/Rerun /||/rerunfilecheck[^.]/{e=e$$0"\n";print red""$$0""end;next}/^LaTeX Warning:/||/natbib Warning:/{w=w$$0"\n";print yel""$$0""end;next}{print}END{if(w||e)print "\n"red"Warning/error summary:\n"byel""w""end;if(e)print red""e""end;exit !!e}'

define basic_latex_rule
  for i in 1 2 3 ; do $(LATEX) $< | $(COLORIZE) && exit 0 ; done ; exit 1
endef

ifeq ($(USEBIBTEX), 1)
define latex_rule
  $(LATEX) $<
  bibtex $*
  $(call basic_latex_rule)
endef
else
define latex_rule
  $(call basic_latex_rule)
endef
endif

.PHONY: all clean

all: $(TARGET).pdf

# dependencies
$(TARGET).pdf: $(DEPENDENCIES)

clean:
	- for e in .tex~ .ps .pdf .dvi .log .toc .nav .out .snm .bbl .blg .spl .lof Notes.bib .maf .fff .lot .ttt ; do rm -f $(TARGET)$$e ; done
	- rm -f *.aux include/*.aux

# general rules
ifeq ($(USEPDFLATEX), 1)
%.pdf %.dvi: %.tex $(DEPENDENCIES)
	$(call latex_rule)

%.ps: %.pdf
	pdf2ps $<
else
%.dvi: %.tex $(DEPENDENCIES)
	$(call latex_rule)

%.pdf: %.ps
	ps2pdf $<

%.ps: %.dvi
	dvips $< -o
endif

# embed pdf fonts
%.embedded_fonts.pdf: %.pdf
	gs -dSAFER -dNOPLATFONTS -dNOPAUSE -dBATCH -sDEVICE=pdfwrite -sPAPERSIZE=a4 -dCompatibilityLevel=1.4 -dPDFSETTINGS=/printer -dCompatibilityLevel=1.4 -dMaxSubsetPct=100 -dSubsetFonts=true -dEmbedAllFonts=true -sOutputFile=$@ -f $<


==> include/na61Abbreviations.tex <==
%%%%%%% units
\newcommand{\kg}{\ensuremath{\mbox{kg}}\xspace}
\newcommand{\eV}{\ensuremath{\mbox{e\kern-0.1em V}}\xspace}
\newcommand{\GeV}{\ensuremath{\mbox{Ge\kern-0.1em V}}\xspace}
\newcommand{\MeV}{\ensuremath{\mbox{Me\kern-0.1em V}}\xspace}
\newcommand{\GeVc}{\ensuremath{\mbox{Ge\kern-0.1em V}\!/\kern-0.07em c}\xspace}
\newcommand{\GeVcc}{\ensuremath{\mbox{Ge\kern-0.1em V}\!/\kern-0.07em c^2}\xspace}
\newcommand{\AGeV}{\ensuremath{A\,\mbox{Ge\kern-0.1em V}}\xspace}
\newcommand{\AGeVc}{\ensuremath{A\,\mbox{Ge\kern-0.1em V}\!/\kern-0.07em c}\xspace}
\newcommand{\MeVc}{\ensuremath{\mbox{Me\kern-0.1em V}\!/\kern-0.07em c}\xspace}
\newcommand{\T}{\ensuremath{\mbox{T}}\xspace}
\newcommand{\cmsq}{\ensuremath{\mbox{cm}^2}\xspace}
\newcommand{\msq}{\ensuremath{\mbox{m}^2}\xspace}
\newcommand{\cm}{\ensuremath{\mbox{cm}}\xspace}
\newcommand{\mm}{\ensuremath{\mbox{mm}}\xspace}
\newcommand{\micron}{\ensuremath{\mu\mbox{m}}\xspace}
\newcommand{\mrad}{\ensuremath{\mbox{mrad}}\xspace}
\newcommand{\ns}{\ensuremath{\mbox{ns}}\xspace}
\newcommand{\m}{\ensuremath{\mbox{m}}\xspace}
\newcommand{\s}{\ensuremath{\mbox{s}}\xspace}
\newcommand{\ms}{\ensuremath{\mbox{ms}}\xspace}
\newcommand{\ps}{\ensuremath{\mbox{ps}}\xspace}
\newcommand{\dd}{\ensuremath{{\mathrm d}}\xspace}
\newcommand{\dedx}{\ensuremath{\dd E\!/\!\dd x}\xspace}
\newcommand{\tof}{\ensuremath{\textup{\textit{tof}}}\xspace}
\newcommand{\pt}{\ensuremath{p_{\mathrm T}}\xspace}
\newcommand{\PT}{\ensuremath{P_\textup{T}}\xspace}
\newcommand{\mT}{\ensuremath{m_{\mathrm T}}\xspace}
\newcommand{\pT}{\ensuremath{p_\text{T}}\xspace}
\newcommand{\pL}{\ensuremath{p_\text{L}}\xspace}
\newcommand{\xF}{\ensuremath{x_\text{F}}\xspace}
\newcommand{\xpF}{\ensuremath{x'_\text{F}}\xspace}
\newcommand{\minv}{\ensuremath{m_\text{inv}}\xspace}


%particles
\newcommand{\pbar}{\ensuremath{\overline{\textup{p}}}\xspace}
\newcommand{\nbar}{\ensuremath{\overline{\textup{n}}}\xspace}
\newcommand{\dbar}{\ensuremath{\overline{\textup{d}}}\xspace}
\newcommand{\pim}{\ensuremath{\pi^-}\xspace}
\newcommand{\pip}{\ensuremath{\pi^+}\xspace}
\newcommand{\km}{\ensuremath{\textup{K}^-}\xspace}
\newcommand{\kp}{\ensuremath{\textup{K}^+}\xspace}
\newcommand{\hm}{\ensuremath{\textup{h}^-}\xspace}

% inverse hyperbolic functions
%\DeclareMathOperator{\acosh}{acosh}
%\DeclareMathOperator{\asinh}{asinh}
%\DeclareMathOperator{\atanh}{atanh}

%%%%%%%%%%%%% some software programs and generators
%----- NA61 software
\def\Offline{\mbox{$\overline{\text%
{Off}}$\hspace{.05em}\raisebox{.4ex}{\underline{line}}}\xspace}
\def\SHOE{\mbox{SHO\hspace{-1.34ex}\raisebox{0.2ex}{\color{green}\textasteriskcentered}\hspace{0.25ex}E}\xspace}
\def\DSHACK{\mbox{DS\hspace{0.15ex}$\hbar$ACK}\xspace}
\DeclareRobustCommand{\SHINE}{\mbox{\textsc{S\hspace{.05em}\raisebox{.4ex}{\underline{hine}}}}\xspace} %DeclareRobustCommand allows this to work in caption
%\def\SHINE{\textsc{Shine}\xspace}
%----- event generators
\def\Glissando{\textsc{Glissando}\xspace}
\newcommand{\FlukaLong}{{\scshape Fluka2008}\xspace}
\newcommand{\FlukaEleven}{{\scshape Fluka2011}\xspace}
\newcommand{\Fluka}{{\scshape Fluka}\xspace}
\newcommand{\UrqmdLong}{{\scshape U}r{\scshape qmd1.3.1}\xspace}
\newcommand{\Urqmd}{{\scshape U}r{\scshape qmd}\xspace}
\newcommand{\GheishaLong}{{\scshape Gheisha2002}\xspace}
\newcommand{\GheishaOld}{{\scshape Gheisha600}\xspace}
\newcommand{\Gheisha}{{\scshape Gheisha}\xspace}
\newcommand{\Corsika}{{\scshape Corsika}\xspace}
\newcommand{\Venus}{{\scshape Venus}\xspace}
\newcommand{\VenusLong}{{\scshape Venus4.12}\xspace}
\newcommand{\GiBUU}{{\scshape GiBUU}\xspace}
\newcommand{\GiBUULong}{{\scshape GiBUU1.6}\xspace}
\newcommand{\FlukaNewLong}{{\scshape Fluka2011.2\_17}\xspace}
\newcommand{\Root}{{\scshape Root}\xspace}
\newcommand{\Geant}{{\scshape Geant}\xspace}
\newcommand{\GeantThree}{{\scshape Geant3}\xspace}
\newcommand{\GeantFour}{{\scshape Geant4}\xspace}
\newcommand{\QGSJet}{{\scshape QGSJet}\xspace}
\newcommand{\DPMJet}{{\scshape DPMJet}\xspace}
\newcommand{\Epos}{{\scshape Epos}\xspace}
\newcommand{\EposLong}{{\scshape Epos1.99}\xspace}
\newcommand{\QGSJetLong}{{\scshape QGSJetII-04}\xspace}
\newcommand{\DPMJetLong}{{\scshape DPMJet3.06}\xspace}
\newcommand{\SibyllLong}{{\scshape Sibyll2.1}\xspace}
\newcommand{\EposLHCLong}{{\scshape EposLHC}\xspace}
\newcommand{\Hsd}{{\scshape Hsd}\xspace}
\newcommand{\Ampt}{{\scshape Ampt}\xspace}

%%%%%%%%%%%%%%%%%%%%%%%% misc
\def\red#1{{\color{red}#1}}
\def\avg#1{\langle{#1}\rangle}
\def\sci#1#2{#1\!\times\!10^{#2}}
\newcommand{\Fi}[1]{Fig.~\ref{#1}}
\newcommand{\CernVM}{\textsc{Cern\-\kern-0.05emVM}\xspace}



==> include/na61Acknowledgments.tex <==
We would like to thank the CERN EP, BE and EN Departments for the
strong support of NA61/SHINE.

This work was supported by the Hungarian Scientific Research Fund (Grants
NKFIH 123842--123959), the J\'anos Bolyai Research Scholarship
of the Hungarian Academy of Sciences, the Polish Ministry of Science
and Higher Education (grants 667\slash N-CERN\slash2010\slash0,
NN\,202\,48\,4339 and NN\,202\,23\,1837), the Polish National Center
for Science (grants~2011\slash03\slash N\slash ST2\slash03691,
2013\slash11\slash N\slash ST2\slash03879, 2014\slash13\slash N\slash
ST2\slash02565, 2014\slash14\slash E\slash ST2\slash00018,
2014\slash15\slash B\slash ST2\slash02537 and
2015\slash18\slash M\slash ST2\slash00125, 2015\slash 19\slash N\slash ST2 \slash01689), the Foundation for Polish
Science --- MPD program, co-financed by the European Union within the
European Regional Development Fund, the Federal Agency of Education of
the Ministry of Education and Science of the Russian Federation (SPbSU
research grant 11.38.242.2015), the Russian Academy of Science and the
Russian Foundation for Basic Research (grants 08-02-00018, 09-02-00664
and 12-02-91503-CERN), the Ministry of Science and
Education of the Russian Federation, grant No.\ 3.3380.2017\slash4.6,
 the National Research Nuclear
University MEPhI in the framework of the Russian Academic Excellence
Project (contract No.\ 02.a03.21.0005, 27.08.2013),
the Ministry of Education, Culture, Sports,
Science and Tech\-no\-lo\-gy, Japan, Grant-in-Aid for Sci\-en\-ti\-fic
Research (grants 18071005, 19034011, 19740162, 20740160 and 20039012),
the German Research Foundation (grant GA\,1480/2-2), the EU-funded
Marie Curie Outgoing Fellowship, Grant PIOF-GA-2013-624803, the
Bulgarian Nuclear Regulatory Agency and the Joint Institute for
Nuclear Research, Dubna (bilateral contract No. 4418-1-15\slash 17),
Bulgarian National Science Fund (grant DN08/11), Ministry of Education
and Science of the Republic of Serbia (grant OI171002), Swiss
Nationalfonds Foundation (grant 200020\-117913/1), ETH Research Grant
TH-01\,07-3 and the U.S.\ Department of Energy.


==> include/na61Authors.tex <==
% based on XML DB with time Fri Aug 11 11:43:06 2017
% Authors in alphabetical order.

\noindent
A.~Aduszkiewicz$^{\,16}$,
Y.~Ali$^{\,13}$,
E.V.~Andronov$^{\,22}$,
T.~Anti\'ci\'c$^{\,3}$,
B.~Baatar$^{\,20}$,
M.~Baszczyk$^{\,14}$,
S.~Bhosale$^{\,11}$,
A.~Blondel$^{\,25}$,
M.~Bogomilov$^{\,2}$,
A.~Brandin$^{\,21}$,
A.~Bravar$^{\,25}$,
W.~Bryli\'nski$^{\,18}$,
J.~Brzychczyk$^{\,13}$,
S.A.~Bunyatov$^{\,20}$,
O.~Busygina$^{\,19}$,
A.~Bzdak$^{\,14}$,
H.~Cherif$^{\,7}$,
M.~\'Cirkovi\'c$^{\,23}$,
T.~Czopowicz$^{\,18}$,
A.~Damyanova$^{\,25}$,
N.~Davis$^{\,11}$,
M.~Deveaux$^{\,7}$,
P.~von~Doetinchem$^{\,30}$,
W.~Dominik$^{\,16}$,
P.~Dorosz$^{\,14}$,
J.~Dumarchez$^{\,4}$,
A.~Datta$^{\,30}$,
R.~Engel$^{\,5}$,
A.~Ereditato$^{\,24}$,
G.A.~Feofilov$^{\,22}$,
Z.~Fodor$^{\,8,17}$,
C.~Francois$^{\,24}$,
A.~Garibov$^{\,1}$,
M.~Ga\'zdzicki$^{\,7,10}$,
M.~Golubeva$^{\,19}$,
K.~Grebieszkow$^{\,18}$,
F.~Guber$^{\,19}$,
A.~Haesler$^{\,25}$,
A.E.~Herv\'e$^{\,5}$,
J.~Hylen$^{\,26}$,
S.N.~Igolkin$^{\,22}$,
A.~Ivashkin$^{\,19}$,
S.R.~Johnson$^{\,28}$,
K.~Kadija$^{\,3}$,
E.~Kaptur$^{\,15}$,
M.~Kie{\l}bowicz$^{\,11}$,
V.A.~Kireyeu$^{\,20}$,
V.~Klochkov$^{\,7}$,
V.I.~Kolesnikov$^{\,20}$,
D.~Kolev$^{\,2}$,
A.~Korzenev$^{\,25}$,
V.N.~Kovalenko$^{\,22}$,
K.~Kowalik$^{\,12}$,
S.~Kowalski$^{\,15}$,
M.~Koziel$^{\,7}$,
A.~Krasnoperov$^{\,20}$,
W.~Kucewicz$^{\,14}$,
M.~Kuich$^{\,16}$,
A.~Kurepin$^{\,19}$,
D.~Larsen$^{\,13}$,
A.~L\'aszl\'o$^{\,8}$,
T.V.~Lazareva$^{\,22}$,
M.~Lewicki$^{\,17}$,
B.~Lundberg$^{\,26}$,
B.~{\L}ysakowski$^{\,15}$,
V.V.~Lyubushkin$^{\,20}$,
M.~Ma\'ckowiak-Paw{\l}owska$^{\,18}$,
B.~Maksiak$^{\,18}$,
A.I.~Malakhov$^{\,20}$,
D.~Mani\'c$^{\,23}$,
A.~Marchionni$^{\,26}$,
A.~Marcinek$^{\,11}$,
A.D.~Marino$^{\,28}$,
K.~Marton$^{\,8}$,
H.-J.~Mathes$^{\,5}$,
T.~Matulewicz$^{\,16}$,
V.~Matveev$^{\,20}$,
G.L.~Melkumov$^{\,20}$,
A.O.~Merzlaya$^{\,22}$,
B.~Messerly$^{\,29}$,
{\L}.~Mik$^{\,14}$,
G.B.~Mills$^{\,27}$,
S.~Morozov$^{\,19,21}$,
S.~Mr\'owczy\'nski$^{\,10}$,
Y.~Nagai$^{\,28}$,
M.~Naskr\k{e}t$^{\,17}$,
V.~Ozvenchuk$^{\,11}$,
V.~Paolone$^{\,29}$,
M.~Pavin$^{\,4,3}$,
O.~Petukhov$^{\,19,21}$,
C.~Pistillo$^{\,24}$,
R.~P{\l}aneta$^{\,13}$,
P.~Podlaski$^{\,16}$,
B.A.~Popov$^{\,20,4}$,
M.~Posiada{\l}a$^{\,16}$,
R.R.~Prado$^{\,5}$,
S.~Pu{\l}awski$^{\,15}$,
J.~Puzovi\'c$^{\,23}$,
R.~Rameika$^{\,26}$,
W.~Rauch$^{\,6}$,
M.~Ravonel$^{\,25}$,
R.~Renfordt$^{\,7}$,
E.~Richter-W\k{a}s$^{\,13}$,
D.~R\"ohrich$^{\,9}$,
E.~Rondio$^{\,12}$,
M.~Roth$^{\,5}$,
B.T.~Rumberger$^{\,28}$,
A.~Rustamov$^{\,1,7}$,
M.~Rybczynski$^{\,10}$,
A.~Rybicki$^{\,11}$,
A.~Sadovsky$^{\,19}$,
K.~Schmidt$^{\,15}$,
I.~Selyuzhenkov$^{\,21}$,
A.Yu.~Seryakov$^{\,22}$,
P.~Seyboth$^{\,10}$,
M.~S{\l}odkowski$^{\,18}$,
A.~Snoch$^{\,7}$,
P.~Staszel$^{\,13}$,
G.~Stefanek$^{\,10}$,
J.~Stepaniak$^{\,12}$,
M.~Strikhanov$^{\,21}$,
H.~Str\"obele$^{\,7}$,
A.~Shukla$^{\,30}$,
T.~\v{S}u\v{s}a$^{\,3}$,
A.~Taranenko$^{\,21}$,
A.~Tefelska$^{\,18}$,
D.~Tefelski$^{\,18}$,
V.~Tereshchenko$^{\,20}$,
A.~Toia$^{\,7}$,
R.~Tsenov$^{\,2}$,
L.~Turko$^{\,17}$,
R.~Ulrich$^{\,5}$,
M.~Unger$^{\,5}$,
F.F.~Valiev$^{\,22}$,
D.~Veberi\v{c}$^{\,5}$,
V.V.~Vechernin$^{\,22}$,
M.~Walewski$^{\,16}$,
A.~Wickremasinghe$^{\,29}$,
C.~Wilkinson$^{\,24}$,
Z.~W{\l}odarczyk$^{\,10}$,
A.~Wojtaszek-Szwarc$^{\,10}$,
O.~Wyszy\'nski$^{\,13}$,
L.~Zambelli$^{\,4}$,
E.D.~Zimmerman$^{\,28}$, and
R.~Zwaska$^{\,26}$


==> include/na61Institutions.tex <==
% based on XML DB with time Fri Aug 11 11:43:06 2017
% Institutes in alphabetical order.

\noindent
$^{1}$~National Nuclear Research Center, Baku, Azerbaijan\\
$^{2}$~Faculty of Physics, University of Sofia, Sofia, Bulgaria\\
$^{3}$~Ru{\dj}er Bo\v{s}kovi\'c Institute, Zagreb, Croatia\\
$^{4}$~LPNHE, University of Paris VI and VII, Paris, France\\
$^{5}$~Karlsruhe Institute of Technology, Karlsruhe, Germany\\
$^{6}$~Fachhochschule Frankfurt, Frankfurt, Germany\\
$^{7}$~University of Frankfurt, Frankfurt, Germany\\
$^{8}$~Wigner Research Centre for Physics of the Hungarian Academy of Sciences, Budapest, Hungary\\
$^{9}$~University of Bergen, Bergen, Norway\\
$^{10}$~Jan Kochanowski University in Kielce, Poland\\
$^{11}$~H. Niewodnicza\'nski Institute of Nuclear Physics of the
      Polish Academy of Sciences, Krak\'ow, Poland\\
$^{12}$~National Centre for Nuclear Research, Warsaw, Poland\\
$^{13}$~Jagiellonian University, Cracow, Poland\\
$^{14}$~AGH - University of Science and Technology, Cracow, Poland\\
$^{15}$~University of Silesia, Katowice, Poland\\
$^{16}$~University of Warsaw, Warsaw, Poland\\
$^{17}$~University of Wroc{\l}aw,  Wroc{\l}aw, Poland\\
$^{18}$~Warsaw University of Technology, Warsaw, Poland\\
$^{19}$~Institute for Nuclear Research, Moscow, Russia\\
$^{20}$~Joint Institute for Nuclear Research, Dubna, Russia\\
$^{21}$~National Research Nuclear University (Moscow Engineering Physics Institute), Moscow, Russia\\
$^{22}$~St. Petersburg State University, St. Petersburg, Russia\\
$^{23}$~University of Belgrade, Belgrade, Serbia\\
$^{24}$~University of Bern, Bern, Switzerland\\
$^{25}$~University of Geneva, Geneva, Switzerland\\
$^{26}$~Fermilab, Batavia, USA\\
$^{27}$~Los Alamos National Laboratory, Los Alamos, USA\\
$^{28}$~University of Colorado, Boulder, USA\\
$^{29}$~University of Pittsburgh, Pittsburgh, USA\\
$^{30}$~University of Hawaii at Manoa, Honolulu, USA\\

